SummerTime: Variable-length Time SeriesSummarization with Applications to PhysicalActivity Analysis

\textit{SummerTime} seeks to summarize globally time series signals and provides a fixed-length, robust summarization of the variable-length time series. Many classical machine learning methods for classification and regression depend on data instances with a fixed number of features. As a result, those methods cannot be directly applied to variable-length time series data. One common approach is to perform classification over a sliding window on the data and aggregate the decisions made at local sections of the time series in some way, through majority voting for classification or averaging for regression. The downside to this approach is that minority local information is lost in the voting process and averaging assumes that each time series measurement is equal in significance. Also, since time series can be of varying length, the quality of votes and averages could vary greatly in cases where there is a close voting tie or bimodal distribution of regression domain. Summarization conducted by the \textit{SummerTime} method will be a fixed-length feature vector which can be used in-place of the time series dataset for use with classical machine learning methods. We use Gaussian Mixture models (GMM) over small same-length disjoint windows in the time series to group local data into clusters. The time series' rate of membership for each cluster will be a feature in the summarization. The model is naturally capable of converging to an appropriate cluster count. We compare our results to state-of-the-art studies in physical activity classification and show high-quality improvement by classifying with only the summarization. Finally, we show that regression using the summarization can augment energy expenditure estimation, producing more robust and precise results.

==> Problem.tex <==
Time series data are a discrete sequence of events of the form $D = \{x_{t_1}, x_{t_2}, \dots ; t_i \in T\}$ such that their index set $T$ is temporal in nature. In many cases, the events do not need to occur at a constant frequency but for the purposes of this paper, we will consider only the case when the time series has events at a constant frequency. 

Classification is the process in which a trained model maps time series data to a nominal class label. Each data point has a true class label associated with it and the ideal classification model will map an instance to its true class label. Traditional classification methods operate on a fixed-length number of features, such that they can be generalized as follows, where $\mathcal D$ is the space of instances each with $k$ features and $\mathcal C$ is the space of class labels.

\begin{equation}
    f(x_1, \dots, x_k) : \mathcal D \to \mathcal C
\end{equation}

For a fixed-length feature vector dataset, we can apply those traditional methods out of the box. In the case of variable-length time series, we cannot apply models of the above form.

One solution to this is to break-up each time series signal into equally-sized time series windows and to perform traditional classification over features of the windows and aggregate a result for the whole through voting, taking the mode. This results in loss of minority information within the signal. In the cases where a signal has equal parts one class and another class, the method observes 50\% confidence in it's classification result. This is akin to a coin flip.

Another solution to this is to rescale the time series signal so that all instances are of the same length. If done through interpolation, estimating and including in-between points, we introduce bias from our choice of interpolation method. In non-smooth signal domains, estimates of in-between points can be radically inaccurate. Regardless of if we account for that bias somehow, rescaling the time series removes proportionality from the signal, relinquishing the distinction between an $n$-second interval and an $m$-second interval. This introduces another bias in that $n$-point intervals are treated equally, even if they correspond to vastly different stretches of real time.

Our first problem is to instead convert variable-length time series data into a fixed-length summarized format so that these summaries will be usable with traditional models. Further, we prefer to do this in a way that preserves global information about the signal (i.e. no data point's contribution is unaccounted for) and preserves in someway proportionality. Finally, we must do this in a data-driven manner to avoid introducing further biases from us, the experimenters.

Our solution is to cluster the time series window features and use the ratios of membership to each cluster as the features of the summary. This fully encapsulates the global information of the signal as the inclusion or exclusion of any point in the signal will change every summary feature. In this way, we can account for proportionality by comparing time series signals of differing lengths without treating their data points as equally frequent. Finally, the summary is constructed using clustering which is unsupervised and does not introduce experimenter bias when assigning points to clusters.

Regression is a similar process to classification in that we are building a model which maps from a data space to a target space. However, the target space is generally numeric and continuous, rather than discrete as in a nominal class space. Regression models are usually of the form:

\begin{equation}
    f(x_1, \dots, x_k) : \mathcal D \to \mathbb R^d
\end{equation}

Again, traditional regression models operate over data with the same number of components. One solution for applying regression models to variable-length data is to treat shorter instances as having missing values. The problem with this is that there are variables which become specifically tuned to long instances from the training set. When presented with new long-instance test data from a different domain distribution, those variables will impact the regression results in ways the training process cannot account for.

Another solution is again to perform the regression locally on windows and aggregate the regression result as a total or average or similar statistic over the windows. In cases where the distribution of windows is multi-modal, an equally-weighted average can push results in the direction of the majority, heavily influenced by the number of points in the signal. This is not ideal as it again introduces the issues of proportionality. However, this influence can be lessened without having to make major changes to the underlying regression model.

In cases where the signals to be regressed over have separate classifications, are different from each other in some categorical way, regression models can be built for each category to produce better results than if a single model was designed to handle every category.

Our solution to this problem is to use the classification result to decide on which regression model to apply to a time series signal. We will apply the regression model to each window and aggregate the result over the whole signal. However, to refine the model, we will include as regression variables the time series summarization of the signal from the clustering. These variables carry information about the signal as a whole which we demonstrate to have a positive effect on time series of differing lengths.

\begin{figure*}
    \centering
    \begin{subfigure}{\textwidth}
    \centering
        \includegraphics[width=0.8\linewidth]{PartZeroWide}
        % AID = 728
        \label{fig:zero}
        \caption{}
    \end{subfigure}
    \begin{subfigure}{0.5\textwidth}
    \centering
        \includegraphics[width=\linewidth]{PartOne}
        \label{fig:one}
        \caption{}
    \end{subfigure}%
    \begin{subfigure}{0.5\textwidth}
    \centering
        \includegraphics[width=\linewidth]{PartTwo}
        \label{fig:two}
        \caption{}
    \end{subfigure}
    \begin{subfigure}{0.5\textwidth}
    \centering
        \includegraphics[width=\linewidth]{ClusterBar}
        \label{fig:three}
        \caption{}
    \end{subfigure}%
    \begin{subfigure}{0.5\textwidth}
    \centering
        \includegraphics[width=\linewidth]{ClusterRatio}
        \label{fig:three2}
        \caption{} 
    \end{subfigure}
    \caption{Above, we show a single instance of Track Running as it makes its way through the clustering phase of the framework. \textbf{(a)} shows the x-axis accelerometer counts for the activity. \textbf{(b)} shows the breakdown of the signal into the 12-second windows for this axis. Not shown is the lag-1 autocorrelation feature. This is the standard means for constructing data instances from physical activity timeseries data. In \textbf{(c)}, we show a PCA projection of the entire activity. The shapes of the data points indicate the clusters each activity window was assigned to. \textbf{(d) and (e)} demonstrate the feature construction from the clustering. The new features associated with an activity instance are the ratios of membership to each cluster.}

    \label{fig:figure1}
\end{figure*} 
